Fast and Scalable Network Slicing by Integrating Deep Learning with Lagrangian Methods

Network slicing is a key technique in 5G and beyond for efficiently supporting diverse services. Many network slicing solutions rely on deep learning to manage complex and high-dimensional resource allocation problems. However, deep learning models suffer limited generalization and adaptability to dynamic slicing configurations. In this paper, we propose a novel framework that integrates constrained optimization methods and deep learning models, resulting in strong generalization and superior approximation capability. Based on the proposed framework, we design a new neural-assisted algorithm to allocate radio resources to slices to maximize the network utility under inter-slice resource constraints. The algorithm exhibits high scalability, accommodating varying numbers of slices and slice configurations with ease. We implement the proposed solution in a system-level network simulator and evaluate its performance extensively by comparing it to state-of-the-art solutions including deep reinforcement learning approaches. The numerical results show that our solution obtains near-optimal quality-of-service satisfaction and promising generalization performance under different network slicing scenarios.

==> authors.tex <==
\author{
\IEEEauthorblockN{Tianlun Hu\IEEEauthorrefmark{1}\IEEEauthorrefmark{3}, 
				  Qi Liao\IEEEauthorrefmark{1}, 
				  Qiang Liu\IEEEauthorrefmark{2}, 
				  and Georg Carle\IEEEauthorrefmark{3}}
\IEEEauthorblockA{ 
	\IEEEauthorrefmark{1}Nokia Bell Labs, Stuttgart, Germany\\
	\IEEEauthorrefmark{2}University of Nebraska Lincoln, United States\\
	\IEEEauthorrefmark{3}Technical University of Munich, Germany\\
Email: \IEEEauthorrefmark{1}\IEEEauthorrefmark{3}\url{tianlun.hu@nokia.com}, 
	   \IEEEauthorrefmark{1}\url{qi.liao@nokia-bell-labs.com}, 
	   \IEEEauthorrefmark{2}\url{qiang.liu@unl.edu},
	   \IEEEauthorrefmark{3}\url{carle@net.in.tum.de}}
	   \vspace{-0.4in}
}
